Odontoceti: Ultra-Fast DAG Consensus with Two Round Commitment

Users of blockchains value scalability, expecting fast confirmations and immediate transaction processing. Odontoceti, the latest in DAG-based consensus, addresses these concerns by prioritizing low latency and high throughput, making a strategic trade-off in security by operating with a 20% fault tolerance instead of the established 33% level. It is the first DAG-based protocol to achieve commitment in just two communication rounds, delivering median latency of 300 milliseconds while processing 10,000 transactions per second under realistic network conditions. Odontoceti operates with n = 5f + 1 validators and creates an uncertified DAG with a novel decision rule for committing blocks. The protocol includes an optimization that advances progress when participants are slow, benefiting crash fault scenarios which are more common in practice than Byzantine faults. Evaluation results demonstrate 20-25% latency improvements compared to an existing production protocol, validating that reducing wave length from three rounds to two rounds yields meaningful performance benefits. This paper establishes the practical viability of lower fault tolerance consensus protocols for blockchains.

==> assets/decide/setup.tex <==
\node[draw=none, anchor=east] at (n1.west) {V1};
\node[draw=none, anchor=east] at (n5.west) {V2};
\node[draw=none, anchor=east] at (n9.west) {V3};
\node[draw=none, anchor=east] at (n13.west) {V4};
\node[draw=none, anchor=east] at (n17.west) {V5};
\node[draw=none, anchor=east] at (n21.west) {V6};

\node[draw=none, anchor=south] at (n1.north) {r1};
\node[draw=none, anchor=south] at (n2.north) {r2};
\node[draw=none, anchor=south] at (n3.north) {r3};
\node[draw=none, anchor=south] at (n4.north) {r4};

% \draw[thick, -, purple] ([yshift=-0.7cm]n21.west) -- ([yshift=-0.7cm, xshift=0.5cm]n22.east) node[draw=none, midway, below, yshift=+0.45cm] {};
% \draw[thick, -, orange] ([yshift=-0.7cm, xshift=-0.5cm]n23.west) -- ([yshift=-0.7cm]n24.east) node[draw=none, midway, below, yshift=+0.45cm] {};
% \draw[thick, -, teal] ([yshift=-1cm, xshift=-0.5cm]n22.west) -- ([yshift=-1cm, xshift=0.5cm]n23.east) node[draw=none, midway, below, yshift=+0.45cm] {};
% \draw[thick, -, brown] ([yshift=-1cm, xshift=-0.5cm]n24.west) -- ([yshift=-1cm]n24.east) node[draw=none, pos=1, right, brown] {\dots};

